Deceptive Patterns of Intelligent and Interactive Writing Assistants

Large Language Models have become an integral part of new intelligent and interactive writing assistants. Many are offered commercially with a chatbot-like UI, such as ChatGPT, and provide little information about their inner workings. This makes this new type of widespread system a potential target for deceptive design patterns. For example, such assistants might exploit hidden costs by providing guidance up until a certain point before asking for a fee to see the rest. As another example, they might sneak unwanted content/edits into longer generated or revised text pieces (e.g. to influence the expressed opinion). With these and other examples, we conceptually transfer several deceptive patterns from the literature to the new context of AI writing assistants. Our goal is to raise awareness and encourage future research into how the UI and interaction design of such systems can impact people and their writing.

==> content/01-intro.tex <==
\section{Introduction}
The increasing role of AI writing tools in writing practices becomes apparent when seeing that millions of people access these tools, such as ChatGPT, everyday. These tools, leveraging recent natural language processing capabilities, are designed to enhance user productivity and communication.
The broad landscape of different AI writing tools, many of which offered commercially however give potential to be prone to deceptive design patterns.

Deceptive design patterns are user interface or user interaction designs that lead the user into taking an action that might not be in their best interest but often in the interest of the third-party designing them. Increasing conversions is often such an interest. \cite{nngroup_deceptive_patterns, Gray2018}

In today's digital landscape, where user engagement and interaction with AI writing assistants are commonplace, the potential for deceptive patterns to influence user behavior is a cause for concern.


By drawing from established deceptive design patterns, such as those identified by Gray et al. \cite{Gray2018}, we aim to extend the understanding of these patterns into the specific context of AI writing tools. We further identified new deceptive design patterns that could be found in AI writing tools.
%
One illustrative example of a deceptive pattern within AI writing tools is the exploitation of \textit{hidden costs}. While users expect assistance in refining their writing, hidden costs emerge when the tool selectively provides suggestions only for a specific paragraph while restricting access to suggestions for the rest of the text. This strategy, as we will elaborate in this paper, serves financial interests, subtly forcing users towards paying for special features and/or subscriptions.

In this paper, we collected examples of the deceptive pattern we have found to possibly exist in AI writing tools. These examples serve as lenses that show how deceptive design patterns might be present in today's AI writing tool and serve for a more nuanced understanding of their potential impact on writers.

==> content/02-background.tex <==
\section{Background \& Related Work}

\subsection{Deceptive (Dark) Patterns}
Design Patterns allow designers to create flexible, elegant, and reusable designs without having to rediscover the design solution themselves over and over again.
This makes them intended to be reused by other practitioners in the future \cite{Gamma1994}.

Design patterns exist in various disciplines: architecture \cite{Alexander1977}, software engineering \cite{Gamma1994}, interface design \cite{Pomeransky1999}, and user experience design \cite{Gray2018}.

Anti patterns are solutions that are commonly used although
they are considered ineffective and potential other proven solutions are existing \cite{Rising1998}.


Dark Patterns in design \cite{Gray2018}.
Dark Patterns of Explainability, Transparency, and User Control for Intelligent Systems \cite{Chromik2019}.

Harry Brignull describes dark patterns as deliberately deceiving users to increase profit within the
limits of law whereas "honest" put users first. \cite{brignull_deception_vs_honesty}


